DreamIdentity: Improved Editability for Efficient Face-identity Preserved Image Generation

While large-scale pre-trained text-to-image models can synthesize diverse and high-quality human-centric images, an intractable problem is how to preserve the face identity for conditioned face images. Existing methods either require time-consuming optimization for each face-identity or learning an efficient encoder at the cost of harming the editability of models. In this work, we present an optimization-free method for each face identity, meanwhile keeping the editability for text-to-image models. Specifically, we propose a novel face-identity encoder to learn an accurate representation of human faces, which applies multi-scale face features followed by a multi-embedding projector to directly generate the pseudo words in the text embedding space. Besides, we propose self-augmented editability learning to enhance the editability of models, which is achieved by constructing paired generated face and edited face images using celebrity names, aiming at transferring mature ability of off-the-shelf text-to-image models in celebrity faces to unseen faces. Extensive experiments show that our methods can generate identity-preserved images under different scenes at a much faster speed.

==> figs/app/style_transfer.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figs/app/style_transfer_fig.pdf}
  \caption{gen}
  \label{fig:style_transfer}
\end{figure}

==> figs/task/task.tex <==
\begin{figure}[tb]
  \centering
  \includegraphics[width=\linewidth]{figs/task/task_fig.pdf}
  \caption{task}
  \label{fig:task}
\end{figure}

==> words.tex <==

# 编辑
editability degradation



scalability and practicality are limited


# 进展
remarkable headway

taken the front in sth



